Shaping the Internet: 10 Years of IXP Growth

Over the past decade, IXPs have been playing a key role in enabling interdomain connectivity. Their traffic volumes have grown dramatically and their physical presence has spread throughout the world. While the relevance of IXPs is undeniable, their long-term contribution to the shaping of the current Internet is not fully understood yet. In this paper, we look into the impact on Internet routes of the intense IXP growth over the last decade. We observe that while in general IXPs only have a small effect in path shortening, very large networks do enjoy a clear IXP-enabled path reduction. We also observe a diversion of the routes, away from the central Tier-1 ASes supported by IXPs. Interestingly, we also find that whereas IXP membership has grown, large and central ASes have steadily moved away from public IXP peerings, whereas smaller ones have embraced them. Despite all this changes, we find though that a clear hierarchy remains, with a small group of highly central networks

==> Makefile <==
.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

PDFLATEX ?= pdflatex
TEX = $(wildcard *.tex) $(wildcard sections/*.tex)

pdf: ixp-hist-conext18.pdf

clean:
	$(RM) figures/*converted-to.pdf *.aux *.log *.out *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

%.pdf: 	$(TEX) $(wildcard *.bib)
	$(PDFLATEX) $*
	-bibtex $*
	if [ -e $*.toc ] ; then $(PDFLATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	$(PDFLATEX) $*


toc: $(wildcard *.tex)
	@egrep -h "\\\((sub)*section|chapter)" $+ | egrep -v "^%" | \
                sed -e 's/\\chapter//;                          \
                s/\\section/    /;                              \
                s/\\subsection/         /;                      \
                s/\\subsubsection/                      /;      \
                s/\\.*{//g;s/[{}]//g' > $@

count:
	texcount -merge ixp-hist-conext18.tex

spellcheck:
	for i in $(TEX); do \
		aspell check --lang=en_US --mode=tex --home-dir=. --dont-backup $$i; \
	done


==> config/packages.tex <==
%!TEX root =  ../main.tex
\usepackage[english]{babel} 
\usepackage{latexsym} % Símbolos
\usepackage{type1cm} % Inclusión de gráficos. Soporte para \figura (más abajo)
%\usepackage[pdftex]{graphicx}
%\usepackage{epstopdf}
%\usepackage{indentfirst}
%\usepackage{amssymb,amsmath,amsthm}
\usepackage{enumitem}
\usepackage{cite}
\usepackage{verbatim}
\usepackage{epsfig}
\usepackage{xcolor}
\usepackage{color}
%\usepackage[a4paper, inner=3.6cm, outer=2.5cm, top=3.5cm, bottom=3.5cm]{geometry}\usepackage{multicol}
\usepackage{subfigure}
\usepackage{xspace}
\usepackage{upgreek}
\usepackage{url}
%\usepackage{slashbox,pict2e}
\usepackage{times}
\usepackage{latexsym}
\usepackage[ruled,noend]{algorithm2e}
\usepackage{ulem} \normalem %to strike out text
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array}
\usepackage{colortbl}
\usepackage{rotating}
\usepackage{changepage}
%\usepackage{fancyvrb}
\usepackage{textcomp}  
%\usepackage{fancyhdr}
\usepackage{marvosym}
\usepackage{setspace}
\usepackage{stfloats}
\usepackage[titletoc]{appendix}
\usepackage{hhline}
\usepackage{afterpage}
\usepackage{lscape}
\usepackage{listings}
\usepackage{caption}
\usepackage{hyperref}
\usepackage[nolist]{acronym}

%remote
%\usepackage{mathtools}
\usepackage{multirow}		
\usepackage{url}
\usepackage{cite}
\usepackage{color}
\usepackage{epstopdf}
%\usepackage{eurosym}
\usepackage{algorithmicx}
%\usepackage[ruled]{algorithm}
\usepackage{algpseudocode}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{eqparbox}
%\usepackage[tight,footnotesize]{subfigure}
\usepackage{import}
%\usepackage{eurosans}
\usepackage{marvosym}
\usepackage{threeparttable}
\usepackage{xcolor}
%\usepackage[titletoc]{appendix}
\usepackage{moresize}

\usepackage{datetime}
\usepackage[linewidth=1pt]{mdframed}
%\usepackage{lipsum}
%\usepackage[super,comma,sort&compress]{natbib} 



==> sections/discussion.tex <==
\section{Limitations}\label{sec:discussion}
%
\paragraph{Traffic volumes.}
While this work focuses on connectivity, we expect that accounting for traffic would strengthen the findings of this paper.
Unfortunately, obtaining a comprehensive and accurate historical traffic dataset is virtually impossible, especially at the scale equivalent to the one considered in this paper. Despite the lack of publicly available data on interdomain traffic, evidence of traffic growth at \ixps does exist. Over the last decade, both large and small \ixps~\cite{chatzis2013there,cardona2012history} have experienced a significant growth in traffic volume exchanged at their facilities. The increased number of traceroutes traversing \ixps implies that the growth in IXP-fabric traffic is not only caused by more traffic flowing on existing routes, but also due to more routes traversing IXPs and thus increasing the traffic throughput. Even when considering connectivity only, we have already seen a more than threefold increase in the number of traces traversing \ixps (see Figure~\ref{fig:traceroute-ixp-non-ixp-filtered-relative-share}). We are confident of the relevance of \ixps in today's Internet.
In particular, the reliance of CDNs on \ixps to deliver their content (such as Netflix~\cite{bottger2018open}) is one of the drivers of this growth. 
Our research shows how \ixps have supported a clear trend of paths reductions to large content providers that confirms earlier observations~\cite{chiu2015we}.
Simultaneously, we also observe an interesting trend by which large and central \ases start avoiding public peering at \ixps from around 2012. This is aligned with the growth of \pnis on the one hand~\cite{Giotsas2017outages}, by which \ases exchanging large  traffic volumes increasingly do so privately, and with the rise of remote peering~\cite{castro2014remote,nomikos2018peer}, which has enable small \ases to join faraway \ixps, making in some cases around one quarter of their membership. 

\gareth{I would remove the above. It's a curve ball - it's lready clear the paper isn't dealing with traffic volumes, so why spend all this space discussing it as a limitation? It would be better to focus on your own real limitations, and push this into a few sexy sentences in future work.}

\paragraph{Data source limitations.}
Unfortunately, it is not possible to observe the Internet completely and accurately at the same time~\cite{willinger2013internet}.
To mitigate these limitations, a large collection of vantage points suitably distributed to maximize visibility is crucial.
We followed this approach by relying on two large historical datasets of traceroutes with different sets of geographically distributed vantage points (see Section~\ref{sec:data-validation}). CAIDA Ark and iPlane complement each other with substantially different vantage points~\cite{huffaker2012internet}. Whereas iPlane relies on vantage points located within academic networks, Ark probes are distributed over a wider variety of network types. While we would have liked to include other data sources (\eg DIMES or Ripe Atlas), since we aimed at obtaining a long historical perspective, we decided to use the two projects with the most available historical data. We also assessed how complete the data's observation capability is in terms of the address space and the \ases covered. This analysis confirmed that most of the Internet is observable through the considered traceroutes. Despite the differences between both platforms, the results derived from them coincide in achieving almost the same conclusions, thus reinforcing our confidence in them.
Additionally, since the popularity of a route on the Internet has been shown to be a proxy for the volume of traffic carried through that route~\cite{sanchez2014inter}, we expect that while visibility of Internet routes is inherently limited, our traceroutes cover those routes likely to represent the greatest traffic volumes.
%

The emergence of \cdns has witnessed different strategies to redirect traffic to caches deep inside other \ases. Unfortunately this is not reflected our data. Problematically, as \cdns have different strategies which might change over time, having comparable longitudinal data is rather challenging. While we acknowledge this as a limitation in our work  we expect that considering this redirectioning  will reinforce our findings towards shorter paths and even less transit dependence. 

Regarding the data on \ixps and their members, the historical nature of our work makes it impossible to rely on active measurements to complete our data. Ideally, we would have liked to complement the existing data with measurements revealing the remoteness of the peers~\cite{castro2014remote} or associating specific links with its corresponding facilities~\cite{Giotsas2015mappingpeering}.
Nevertheless, we are confident that PeeringDB provides a rich enough snapshot of the \ixp ecosystem~\cite{bottger2018looking,lodhi2014using}.

\gareth{I find the above a bit defensive, and it kinda undermines the previous story. I would put it early on in the paper. Conciselt deal with the issue, and then move onto the analysis. Allocating all this space makes the paper look weak.}

\paragraph{Generality of the results.}
As discussed in the previous paragraph, observing the Internet as a whole is a very challenging task.
We openly acknowledge that our dataset cannot cover all networks and prefixes for every point in time over the last ten years.
It is certain that there are singular examples of networks or prefixes that exhibit significantly different changes than the ones highlighted in this paper. We nevertheless argue that the aim of this paper is not to infer individual cases of path shortening or flattening, but to develop a holistic understanding of the phenomenon. 
%If shortening was a wide-spread phenomenon impacting a majority of paths, we would have expected to observe at least some shortening over time.

Our results reinforce the idea that Internet flattening and path shortening are too different concepts.
As far as we can infer through our dataset, \ixps have a general hierarchical flattening effect, helping most \ases to bypass T1 transit providers. Differently, the impact of \ixps on path shortening tends to be focused on hypergiants.
From a traffic perspective though, this is likely to imply that most Internet traffic has enjoyed significant path shortening.

\gareth{I would also kill the above. It comes too late in the paper, and you spend to much space on it. It really inflates the idea that the paper is flawed...}

%While this might improve latency or throughput and save costs on transit providers, it does not necessarily lead to path shortening over time. However, it is true that in general paths through IXPs are shorter than pure-transit paths, which implies that shifting traffic from purely-transit to IXPs creates the perception of paths becoming shorter.

%In this paragraph I would want to talk about to which extent our results hold for the whole Internet, reflecting the still to be done data validation part.
%The final point here would be that yes, our data has severe limitations, but we made exhausitvely sure that all destinations of importance are covered.
%And yes, we do not see everything, but we are still very confident that the analysis carried out in this paper sharpens the understanding of the differences between flattening and shortening.

%\paragraph{Limited data availability}
%We could have included more traceroute data sources into the paper as well, like DIMES, Ripe Atlas (and all the others, list exhaustively).
%However, since we were interested in a historic perspective, we chose to use the two with the longest reaching history \todo{T: No clue whether this is true, making up stuff out of thin air here}
%The final point here would be that yes, our data is limited, but is is quite likely the best one we will ever get (until time travel is invented).


==> sections/traces.tex <==
\section{On the Routes Through IXPs}\label{sec:traces}

\gareth{Not sure I get the title - because this section is dataset description, right? Could we introduce the word dataset to the title?}

In the previous section we analyzed the evolution of the \ixp ecosystem over time. This evolution shows a 
growth in terms of facilities and members, resulting in large gains in terms of reachability, with around 
80\% of the announced address space by 2016. Since these changes are likely to have a significant impact on 
the Internet end-to-end paths, in this section we study how Internet routes have evolved and how 
\ixps have supported this evolution.


\subsection{Dataset Description}
\label{sec:ixp-dataset}

%\gareth{Minor point: we switch between past/present/past present tense. I've tried to standardize, but may have missed some...}

We use two different datasets of traceroutes spanning over a decade: (1) The iPlane 
project~\cite{madhyastha2006iplane} includes traceroutes launched from 
PlanetLab nodes to addresses in all the routable prefixes from the year 2006 
to 2016, and (2) CAIDA Ark~\cite{caida-traceroute} includes traceroutes from Ark 
monitors to randomly selected destinations for each routed IPv4 /24 prefix 
on the Internet since 2007. iPlane and Ark complement each other: 
while iPlane vantage points are usually located within academic networks, 
Ark traces originate from a wider variety of networks. We use all available data from the iPlane 
project (June 2006 to August 2016) and a similar timeframe (October 2007 to August 2016) 
from Ark\footnote{There is no Ark data prior to October 2007.}.
We aim at using time-aligned snapshots in a monthly fashion. For iPlane we 
use, whenever possible, the snapshots taken on the first of each month. Similarly, 
for Ark, we use all measurement cycles covering the first of each month, or if no snapshot
is available that day, we use the previous or next day if available.
Note that iPlane suffered a large outage with no data available between November 2010 
and July 2011. Other than this, there are only four months for which we could 
not find an iPlane snapshot. As these months are non-consecutive, we expect 
limited impact on the provided results. In the case of Ark, we could find snapshots 
for all months expect one. In total, we use snapshots from 109 different months 
for iPlane and 107 for Ark.

\subsection{Data Validation}
\label{sec:data-validation}
This section assesses the coverage and bias of our traceroute datasets.
Specifically, we look at the geographic coverage of the measurement sources 
as well as their targeted destinations. 
%Table~\ref{tab:probe-overview}
%provides a high-level comparison of the two measurement platforms
%used, i.e., iPlane and Caida Ark.
% Steve: If we do not provide the AS-level bias somewhere else,
% then we have to do it here. Either would be fine. 

% Steve: the table below is rather useless in terms of space usage.
%Ign: killed
%\begin{table}
%	\centering
%	\begin{tabular}{l|ll}
%		\toprule
%		~ & iPlane & Ark \\
%		\midrule
%		Number of probes & 1,218  & 171 \\
%		Probes per snapshot & 157.8 & 56.0 \\
%		Deployment Mode & PlanetLab & Single Nodes \\
%		First data & 06/2006 & 09/2007 \\
%		Last data & 08/2016 & ongoing \\
%		\bottomrule
%	\end{tabular}
%	\caption{Comparison between iPlane and Caida Ark.}
%	\label{tab:probe-overview}
%\end{table}

\gareth{Does sanitization belong here? This isn't validation, it's pre-processing? Perhaps move into previous subsection?}
\paragraph{Sanitization of traceroutes.}
The selected snapshots contain more than 6.7 billion individual traceroutes, 2.3 
billion from iPlane and 4.4 billion from CAIDA Ark. To ensure the reliability of our 
results, we followed a three step approach, applying 3 filters on the dataset. 

%%
%\noindent \textit{Step 1: destination AS filter}. To avoid underestimating the length of a path 
%in the Internet, we require that each traceroute contains a reply from the destination AS.
%This invalidates 3.9 billion Ark traceroutes and 930 million iPlane traceroutes. We also find that 
%496 Ark traceroutes and a whopping 8.2 million iPlane traceroutes contain more than one reply from the 
%destination IP\footnote{These iPlane traceroutes do not terminate, sending unnecessary probes, 
%	while we can see an answer from the destination.}, within the same snapshot. We only keep traceroutes 
%containing exactly one reply from the destination IP. \ignacio{Do we still do so now that we have moved to filter on destination AS instead of IP} After applying this filter, we have 503 million 
%traces (11.4\%) for Ark and 1.4 billion (60.4\%) for iPlane. 
%
%\noindent \textit{Step 2: Unresolved hop filter}. We further require that no more than one consecutive hop is 
%unresolved. In entering and exiting an \as, a traceroute will typically exhibit (at least) 
%two IP hops. Therefore, we consider this unique unresolved IP hop criteria to prevent cases where multiple unresolved
%hops would actually be an additional \as.
%This steps discards 141k (3.2\%) and 321k (13.6\%) of Ark iPlane traceroutes respectively.
%
%\noindent \textit{Step 3: Single \ixp filter}. Finally, we require that traceroutes do not contain more than 
%one \ixp crossing. In conformance with valley-free routing expectations, we assume that 
%there should not be more than one peering relationship on a given path. Therefore, for safety, 
%in the few cases where we observe more than one \ixp, we discard the traceroute. While valley-free 
%routing violations happen~\cite{giotsas2012valley}, this filter eliminates less than 15k 
%traces, \ie below 1\% of the traces of each data set.

\gareth{Minor, but the below look like paragraphs, so it breaks the structure. Could we perhaps change the paragraph format to bold rather than just italics?}

\noindent \textit{Step 1: destination IP filter}. To avoid underestimating the length of a path 
in the Internet, we require that each traceroute contains a reply from the destination IP.
This invalidates 3.9 billion Ark traceroutes and 930 million iPlane traceroutes. We also find that 
496 Ark traceroutes and 8.2 million iPlane traceroutes contain more than one reply from the 
destination IP\footnote{These iPlane traceroutes do not terminate, sending unnecessary probes, 
while we can see an answer from the destination.}, within the same snapshot. We only keep traceroutes 
containing exactly one reply from the destination IP. After applying this filter, we have 503 million 
traces (11.4\%) for Ark and 1.4 billion (60.4\%) for iPlane.

\noindent \textit{Step 2: Unresolved hop filter}. We further require that no more than one consecutive hop is 
unresolved. In entering and exiting an \as, a traceroute will typically exhibit (at least) 
two IP hops. Therefore, we consider this unresolved IP hop to prevent cases where this unresolved
hop would actually be an additional \as on the path and would not be accounted for.
This steps discards 141k (3.2\%) and 321k (13.6\%) of Ark iPlane traceroutes respectively.

\noindent \textit{Step 3: Single \ixp filter}. Finally, we require that traceroutes do not contain more than 
one \ixp crossing. In conformance with valley-free routing expectations, we assume that 
there should not be more than one peering relationship on a given path. Therefore, for safety, 
in the few cases where we observe more than one \ixp, we discard the traceroute. While valley-free 
routing violations happen~\cite{giotsas2012valley}, this filter eliminates less than 15k 
traces, \ie below 1\% of the traces of each data set.

After the complete sanitization process (summarized in Table~\ref{tab:dataset-sizes}), we 
end up with 358M Ark and 1.1 billion iPlane traces, representing 8.1\% and 46.1\% of the 
initial data sets, respectively. 

\begin{table}
	\centering
	\begin{tabular}{l|rr|r}
		\toprule
		~ & iPlane & Ark & total \\
		\midrule
		All traceroutes & 2.3B & 4.4B & 6.7B \\
		Step 1: Destination IP filter & 1.4B & 503M & 1.9B \\
		Step 2: Unresolved hop filter  & 1.1B & 362M & 1.5B \\
		Step 3: Single \ixp filter & 1.1B & 358M & 1.5B \\
		\bottomrule
	\end{tabular}
	\caption{Sizes of the datasets, before and after the sanitization process.}
	\label{tab:dataset-sizes}	
\end{table}

% We are confident that our traceroute dataset provides sufficient coverage: after this thorough sanitation, the remaining traceroutes cover most of the announced address space with more than half of the \ases present in the global routing table representing more than 82\% of the announced IPv4 space. 
% But how much of the AS relationships do we lose by doing this? Same for IP and AS reachability.

We are confident that our traceroute dataset provides sufficient coverage:
In the following pargraphs, we show that the data collected has a sufficient coverage of the Internet in terms of (1) geographical regions, (2) prefixes and (3) \ases and IPs. We also verify that our sanitation steps do not significantly reduce or bias the coverage provided by the data.

%\paragraph{CAIDA Ark vs. iPlane.}
%CAIDA Ark and iPlane have substantially different vantage points and therefore provide different views of the Internet. Whereas iPlane relies on vantage points located within academic networks, Ark probes are distributed over a wider variety of network types. Despite of this and other differences~\cite{huffaker2012internet}, both platforms coincide in achieving almost exactly the same conclusions, reinforcing our confindence on them.
%We now show in Figure/Table the differences over the years in terms of 
%\todo{Maybe a paragraph in the discussion on the validity of results showing the differences between the 2 datasets across some of the main metrics used}

%origin and destinations of the traceroutes. \todo{currently we don't}
%While the former can be easily obtained by knowing the origin node, 
%for the latter we use Maxmind\footnote{https://www.maxmind.com/en/home}. 
%As we are mostly interested on a higher level of aggregation, \ie 
%continent level, the known limitations of IP geolocation (particularly 
%significant below the country level~\cite{geolo6081357}) are unlikely 
%to be relevant in this case. For the geolocation of \ixps, we directly 
%leverage the information contained in PeeringDB, so we expect here a 
%high level of accuracy.

\paragraph{Geographic Probe Coverage}
Before continuining, it is important to quantify the geographical coverage and bias contained without dataset. 
Since PlanetLab does neither encode countries into hostnames directly nor provides historic 
information on decommissioned nodes, we cannot automatically obtain location 
information for all iPlane nodes. Where available, we instead use the Top Level Domain (TLD) of the 
PlanetLab node name to infer the country where the node is/was located (\eg
\textit{planet-lab1.itba.edu.ar} or \textit{planetlab1.itwm.fhg.de}). This is 
feasible for 657 (54\%) PlanetLab nodes. Out of the remaining 561 PlanetLab nodes, 
a majority of 384 domain names map to the .edu TLD, which in most cases
maps to US universities. In cases where we could not rely on the TLD, we resolve 
names to countries manually. While the resolution in most cases was 
straightforward (\eg \textit{planetlab-1.cs.princeton.edu}), it sometimes
required more manual inspection (\eg \textit{plab1.create-net.org} appears to be 
an Italian node). We sanitized data to the best of our knowledge, but cannot rule out small issues. Nevertheless, we have high confidence in at least the mapping of country-specific TLDs and the .edu TLD, which corresponds to more 
than 85\% of all node names. As for Caida Ark, the mapping of nodes to 
countries could be derived automatically, since all Ark nodes embed the 
TLD of the countries in the node name.

Table~\ref{tab:probes-continents} shows the distribution of measurement nodes with
respect to continents: Europe, Asia and Africa dominate. However, to 
put values into the right perspective, in the total column we also denote how many 
countries of a continent are covered by iPlane and Caida Ark and provide the respective 
percentages in the table  (column ``\% Cnt''). We see that while Europe is well covered, in terms 
of relative coverage, South America is performing better than Africa and Asia. To get 
a better understanding of which countries within a continent are covered, we also assess which 
fraction of a continent's population the covered countries represent (column ``\% Pop.'').
At least half of the population in each continent has a measurement probe 
deployed in their country. Specifically, North America and Asia achieve more than 80\% 
coverage, followed by South America and Oceania with more than 70\% each. Europe achieves 
more than 60\% coverage while only Africa gets less than 60\% coverage. Coverage 
appears to be in line with the development status of continents, with a bias towards 
better coverage for more developed regions. 

\gareth{Any insight into the geo coverage of the traceroute targets?}

\begin{table}
	\centering
	\begin{tabular}{l|rr|r|r|r}
		\toprule
		Continent & iPlane & Ark & Total & \% Cnt. &  \% Pop. \\
		\midrule
		Africa & 2 & 14 & 16 of 58 & 27.6\% & 53.1\% \\
		Asia & 13 & 12 & 17 of 58 & 29.3\% & 82.9\% \\
		Europe & 22 & 23 & 27 of 57 & 47.4\% & 66.1\% \\ 
		North America & 5 & 4 & 5 of 43 & 11.6\% & 87.7\% \\
		Oceania & 2 & 2 & 2 of 27 & 7.4\% & 73.8\% \\
		South America & 6 & 3 & 6 of 14 & 42.9\% & 76.1\% \\
		\bottomrule
	\end{tabular}
	\caption{Countries per continent in which a probe is hosted for both platforms.}
	\label{tab:probes-continents}
\end{table}

%Table~\ref{tab:probes-countries} lists for each measurement platform the ten countries 
%with most probes installed. Besides a dominance of more developed countries and a bias 
%towards Western countries, we also see that iPlane used significantly more probes per 
%country than Caida. 

%\begin{table}
%	\centering
%	\begin{tabular}{l|lr|lr}
%		\toprule
%		~ & \multicolumn{2}{c|}{iPlane} & \multicolumn{2}{c}{Ark} \\
%		\midrule
%		1 & US & 486 & US & 48 \\
%		2 & DE & 87 & DE & 8 \\
%		3 & CN & 55 & SE & 7 \\
%		4 & FR & 49 & CA & 6 \\
%		5 & JP & 44 & NL & 6 \\
%		6 & CA & 42 & CN & 5 \\
%		7 & GB & 41 & AU & 5 \\
%		8 & PL & 35 & FR & 5 \\
%		9 & IT & 32 & IT & 4 \\ 
%		10 & ES & 26 & ES & 4\\
%		\bottomrule
%	\end{tabular}
%	\caption{Top 10 countries with most probes deployed for iPlane and Ark platforms.}
%	\label{tab:probes-countries}
%\end{table}

\begin{figure*}
	\begin{subfigure}{\columnwidth}
		\includegraphics[width=\columnwidth]{graphs/coverage-as-ips-pref-ipla}
		\caption{iPlane}
	\end{subfigure}
	\begin{subfigure}{\columnwidth}
		\includegraphics[width=\columnwidth]{graphs/coverage-as-ips-pref-ark}
		\caption{Caida Ark}
	\end{subfigure}
	\caption{Number of prefixes and ASes  (in thousands) and prefix size and the number of IPs (in billions), in the global routing table (\textit{``Total''}), in each dataset (\textit{``Step 0''}) before sanitization, and after sanitization (\textit{``Step 3''}).}
	\label{fig:bias}
\end{figure*}

\paragraph{Prefix Coverage}
To determine which part of the Internet is covered by our traceroute dataset, we first look at 
the prefixes targeted by the traceroutes. Taking as reference all the prefixes in the global routing 
table, as extracted from CAIDA's routeviews data~\cite{caida-routeviews}, we consider only those prefixes not 
longer than /24 -- in accordance with the best BGP practice, that discourages the usage of longer prefixes. 
We count the number of matching prefixes, \ie all the prefixes matching the destination IP of a specific traceroute, 
not just the most specific one.

Figure~\ref{fig:bias} (top four plots) shows for (1) iPlane and (2) Ark, the number of prefixes (in thousands) and the size of the IP space those prefixes represent (in billions of IPs).
The prefixes of the global routing table are marked as \textit{``Total''}.
The prefixes covered by the original traceroute datasets (\textit{``Step 0''}) are also shown as well as the prefixes that remain after applying the 3 sanitization filters mentioned above (\textit{``Step 3''}).
While iPlane on average only covers 36\% of the announced prefixes, Ark on average achieves a coverage of 96\% of all announced prefixes.
For iPlane the coverage drops to 29\% after sanitization, whereas for Ark due to the bigger number of traceroutes removed, coverage drops to 36\%.
Overall, the two platforms together cover roughly 50\% of the total prefixes, indicating some overlap in the target selection (not shown in the plots).

%Caida Ark constantly covers between 30\% and 40\%, depending on whether less specifics prefixes are considered.
%In contrast, iPlane achieves a lower coverage of between 20\% and 30\% of the prefixes, exhibiting a decay over time, which then suddenly improves before decaying again.
%We expect that this behaviour is caused by the target update strategy which achieves higher coverage after an update, but then decreases as the Internet grows.

%\begin{figure}
%	\includegraphics[width=\columnwidth]{graphs/fraction-prefix-traceroute}
%	\caption{Fraction of prefixes of the global routing table targeted by traceroutes.}
%	\label{fig:pfx-covered}
%\end{figure}

The prefixes targeted by iPlane and Caida Ark account for 63\% and 97\% of the announced IP space respectively. 
We reach this percentage by considering the prefix coverage and comparing with the total number of IP addresses announced in the global routing table.
After our sanitization, coverage drops to 52\% and 63\% respectively.
However, when combined, the two platforms still probe prefixes accounting for roughly 80\% of the announced IP space

%\begin{figure}
%	\includegraphics[width=\columnwidth]{graphs/fraction-IP-traceroute}
%	\caption{Fraction of IPs of the global routing table targeted by traceroutes.}
%	\label{fig:pfx-covered-size-ip-space}
%\end{figure}

\paragraph{AS and IP Coverage.}
We now examine our coverage in terms of \ases and IPs.
We consider an AS to be covered if at least one of its IPs is targeted by a traceroute. We map IPs to \ases using~\cite{caida-routeviews}.
Similarly to the previous case, Figure~\ref{fig:bias} (bottom four plots) shows for (a) iPlane and (b) Ark, all the \ases (in thousands) and the IPs (in billions) present in the global routing table (\textit{``Total''}), the \ases and IPs seen by the corresponding traceroute dataset (\textit{``Step 0''}), as well as the \ases and IPs remaining after the sanitization process (\textit{``Step 3''}).
The two platforms independently cover 50\% to 70\% of the total ASes, while their union covers more than 80\%. 
As for the previous case, we also investigated the amount of the IP address space that the covered ASes represent. Specifically, we found that the ASes targeted by both platforms announce more than 90\% of the global IPv4 space.


In the following, unless stated otherwise, we will always only show results obtained from the CAIDA Ark measurements in all Figures and calculations.
In all the analysis steps we carry out, the two platforms consistently yielded results so similar, that for the sake of clarity in the plots, we decided to only show one of the platforms.
We believe that this similarity in the results obtained through two different, independent measurement platforms strongly reinforces the validity of the results.


\gareth{It would be nice to have a clear conclusion here that explains what bias actually exists. What are the key points the reader should remember when reading the rest of the paper?}

%\begin{figure}
%	\begin{subfigure}{0.49\columnwidth}
%		\includegraphics[width=\columnwidth]{graphs/traceroute-coverage-as}
%		\caption{ASes covered by traces}
%	\end{subfigure}
%	\begin{subfigure}{0.49\columnwidth}
%		\includegraphics[width=\columnwidth]{graphs/traceroute-coverage-ip}
%		\caption{AS IP space covered}
%	\end{subfigure}
%	\caption{Fraction of ASNs and AS IP space covered by traceroutes.}
%	\label{fig:traceroute-asn-coverage}
%\end{figure}




%We now look at the growth in the number of peerings as well as whether these take place at \ixps or not.
%Figure~\ref{fig:in-vs-out-ixp-peerings} shows how the number of peerings has substantially grown over the years and how such growth has been supported by \ixps. We infer an upper bound of peering connections at \ixps by considering colocated \ases that happen to be peering (according to our \ixp and \ases-relationships datasets, see Section~\ref{sec:reachability}), as doing so at such facility.
%% where do we show the ratio? don't see any figure doing this (Figure 8 is the one i thought is relevant here)
%A ratio close to one between the total number of peerings and those that take place at \ixps illustrates how much peering is indeed facilitated by the emergence of \ixps. Despite the growing relevance of \ixps, private peering outside of exchange points is still popular. Note that while private peerings at \ixps might be  also common, we cannot identify with our data whether in-\ixp peerings are public or private.
%
%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{graphs/evolution_peerings}
%	\caption{Evolution of the number of the potential peerings at IXPs and outside them.}
%	\label{fig:in-vs-out-ixp-peerings}
%\end{figure}

%\subsection{Routes through the \ixps}
%To understand the role of \ixps on Internet routes, we first examine whether \ixps have actually increasingly attracted routes over time.
%We now identify \ixps crossings 
%with the traIXroute tool~\cite{nomikos2016traixroute} using the datasets described before (see Section~\ref{sec:data-validation}).
%We find that out of the total of 1.45 billion traceroutes, 1.2 billion (86\%) do not traverse an \ixp whereas the remaining 
%206 million (14\%) do. On average, there are 2.8M non-\ixp and 513k traceroutes in the Caida 
%Ark dataset and 8.6M non-\ixp and 1.4M \ixp in the iPlane one. Table~\ref{tab:dataset-overview} 
%provides a more detailed breakdown of the composition of the data set.

% We need more details in this table, it's way too high-level summary. I'd like to see for each filter
% the reduction in AS-level coverage (and IP coverage) to show the bias from the sanitization process.
%\begin{table}
%	\centering
%	\begin{tabular}{l|rr|r}
%		\toprule
%		~ & iPlane & Ark & ~ total\\
%		\midrule
%		IXP traces & 151.2M & 54.9M & 206.1M \\
%		non-IXP traces& 941.4M & 303.2M & 1,244.6M \\
%		total & 1,092.6M & 358.0M & 1,450.6M\\
%		\midrule
%		Timestamps & 109 & 107 & - \\
%		\bottomrule
%	\end{tabular}
%	\caption{Traceroute Dataset Overview.}
%	\label{tab:dataset-overview}
%\end{table}

%Figure~\ref{fig:traceroute-ixp-non-ixp-filtered-relative-share} shows the evolution of the relative share of traceroutes that traverse \ixps.
%We observe a linear and clear, although not strongly pronounced, trend towards a larger fraction of traceroutes going through IXPs.
%While in 2008 only about 6\% of the traces in a snapshot traversed an IXP, by 2016 the share had more than tripled with about 20\% of all the traces going through an IXP\footnote{The careful reader will have noticed that the behaviour in 2007 might suggests that in that period the share of traceroutes going through IXPs has actually decreased. When inspecting this period before 2008, it appears that it is actually the number of non-IXP traceroutes that has dropped in absolute value, likely due to a measurement artifact, therefore showing up as an increase of IXP traceroutes.}.

%While this might seem a relatively moderate change, we want to emphasise that those figures only reflect connectivity. 
%Overall, a more than threefold increase in the number of traces traversing an IXP purely based on connectivity, is a strong indicator that IXPs are becoming a more and more important interconnection facility in today's Internet. We discuss in Section~\ref{sec:discussion} how accounting for traffic volumes is likely to amplify the observed trends.


